Asymptotically optimal quantization schemes for Gaussian processes

We describe quantization designs which lead to asymptotically and order optimal functional quantizers. Regular variation of the eigenvalues of the covariance operator plays a crucial role to achieve these rates. For the development of a constructive quantization scheme we rely on the knowledge of the eigenvectors of the covariance operator in order to transform the problem into a finite dimensional quantization problem of normal distributions. Furthermore we derive a high-resolution formula for the $L^2$-quantization errors of Riemann-Liouville processes.

==> applications.tex <==
\section{Applications for Functional Quantization of the Brownian motion}
From the knowledge of quantizers of the Brownian motion and the 
weights of the corresponding Voronoi cells $\left(\Prob(W \in
C_g(\gamma))\right)_{g\in\gamma}$ a cubature formula for functionals of $\hat W$
is straightforward, i.e.
\[
	\E \Psi(\widehat W^\gamma) = \sum_{g\in\gamma} \Prob_W \bigl(C_g(\gamma)\bigr) \Psi(g)
\]
for a $\Psi: L^2([0,T],dt) \to \mathbb{R}$.
This can be even extended to the quantization of diffusions under some
assumptions on the diffusion coefficient (see \cite{diffusions}).
Hence it is possible to apply functional quantization of the Brownian Motion to
problems of mathematical finance driven by diffusion processes\ldots



==> biblio.tex <==
\begin{thebibliography}{99}
\bibitem{BOPA} Bouton C., Pag\`es G., About the multi-dimensional Competitive Learning Vector
Quantization Algorithm with constant gain, {\em Ann. Applied Probab.}, {\bf 7} (3) (1997), 670-710.

\bibitem{DERE}
Dereich, S., {\em High resolution coding of stochastic processes and small ball probabilities}, PhD thesis, TU Berlin, 2003.
%
\bibitem{DONO}
Donoho, D.L., {\em Counting bits with Kolmogorov and Shannon}, Technical Report 38, Stanford University, 2000.
%
\bibitem{GERSH}
Gersho, A., Gray, R.M., {\em Vector Quantization and Signal Compression}. Kluwer, Boston, 1992.
%
\bibitem{GRALU1}
Graf, S., Luschgy, H., {\em Foundations of Quantization for Probability Distributions}, Lecture Notes in Mathematics, Vol.
1730, Springer, Berlin, 2000.
%
\bibitem{GRALU2}
Graf, S., Luschgy, H., The point density measure in the quantization of self-similar probabilities, {\em Math. Proc. Cambridge Phil. Soc.}, (to appear).
%
\bibitem{GRALU3}
Graf, S., Luschgy, H., Sharp asymptotics of the metric entropy for ellipsoids, {\em J. Complexity}, {\bf  20} (2004), 876-882.
%
\bibitem{GRAY}
Gray, R.M., Neuhoff, D.L., Quantization, {\em IEEE Trans. Inform.}, {\bf  44}, (1998) 2325-2383.
%
\bibitem{KOLMO}
Kolmogorov, A.N., Tikhomirov, V.M., $\varepsilon$-entropy and $\varepsilon$-capacity of sets in functional
spaces, {\em Amer. Math. Soc. Transl. Ser.}, {\bf  2}(17) (1961), 272-364.
%
\bibitem{LUPA1}
Luschgy, H., Pag\`es, G., Functional quantization of stochastic processes, {\em J. Funct. Anal.}, {\bf  196}  (2002), 486-531.
%
\bibitem{LUPA2}
Luschgy, H., Pag\`es, G., Sharp asymptotics of the functional quantization problem for Gaussian processes, {\em Ann.
Probab.}, {\bf 32} (2004), 1574-1599.
%
\bibitem{LUPA3}
Luschgy, H., Pag\`es, G., Sharp asymptotics of the Kolmorogov entropy for Gaussian measures, {\em J. Funct. Anal.}, {\bf 212}  (2004), 89-120.
%
\bibitem{LUPA4}  Luschgy, H., Pag\`es, G., Functional quantization of 1-dimensional Brownian
diffusions, Preprint. LPMA Universit\'e Paris 6, 853, 2003.

\bibitem{PAGE1}
Pag\`es, G., A space vector quantization method for numerical integration, {\em J. Computational and Applied Math.}, {\bf 89} (1997), 1-38.
%
\bibitem{PAPRIN}
Pag\`es, G., Printems, J., Optimal quadratic quantization for numerics: the Gaussian case, {\em Monte Carlo Methods and Applications},
{\bf  9} (2003), 135-166.
%
\bibitem{PAGE2}
Pag\`es, G., Pham, H., Printems, J., Optimal quantization methods and applications to numerical methods and applications in finance,
{\em Handbook of Computational and Numerical Methods in Finance} (ed. S. Rachev), 253-298, Birkh{\"a}user, 2004.
%
\bibitem{PAGE3}
Pag\`es, G., Printems, J., Functional quadratic quantization for pricing derivatives, Preprint LMPA 930, Universit{\'e} Paris 6, 2004.
%
\bibitem{TUAN}
Vu Kim Tuan, Gorenflo, R., Asymptotics of singular values of Volterra integral operators, {\em Numer. Funct. Anal. and Optimiz.}, {\bf 17} (1996), 453-461.
%
\bibitem{WILB}
Wilbertz, B., Work in progress, 2004.
\end{thebibliography}
